Detecting Temporal Correlation via Quantum Random Number Generation

All computing devices, including quantum computers, must exhibit that for a given input, an output is produced in accordance with the program. The outputs generated by quantum computers that fulfill these requirements are not temporally correlated, however. In a quantum-computing device comprising solid-state qubits such as superconducting qubits, any operation to rest the qubits to their initial state faces a practical problem. We applied a statistical analysis to a collection of random numbers output from a 20-qubit superconducting-qubit cloud quantum computer using the simplest random number generation scheme. The analysis indicates temporal correlation in the output of some sequences obtained from the 20 qubits. This temporal correlation is not related to the relaxation time of each qubit. We conclude that the correlation could be a result of a systematic error.

==> eptcsdata.tex <==
\providecommand{\firstpage}{18}
\providecommand{\publicationstatus}{G. Di Molfetta, V. Kendon \& Y. Shikano (Eds.): 9th International\\ Conference on Quantum Simulation and Quantum Walks (QSQW 2020)\\
EPTCS 315, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.315.2}{10.4204/EPTCS.315.2}}
\pdfoutput=1

